Discrete time optimal control with frequency constraints for non-smooth systems

We present a Pontryagin maximum principle for discrete time optimal control problems with (a) pointwise constraints on the control actions and the states, (b) frequency constraints on the control and the state trajectories, and (c) nonsmooth dynamical systems. Pointwise constraints on the states and the control actions represent desired and/or physical limitations on the states and the control values; such constraints are important and are widely present in the optimal control literature. Constraints of the type (b), while less standard in the literature, effectively serve the purpose of describing important spectral properties of inertial actuators and systems. The conjunction of constraints of the type (a) and (b) is a relatively new phenomenon in optimal control but are important for the synthesis control trajectories with a high degree of fidelity. The maximum principle established here provides first order necessary conditions for optimality that serve as a starting point for the synthesis of control trajectories corresponding to a large class of constrained motion planning problems that have high accuracy in a computationally tractable fashion. Moreover, the ability to handle a reasonably large class of nonsmooth dynamical systems that arise in practice ensures broad applicability our theory, and we include several illustrations of our results on standard problems.

==> flowchartproof.tex <==
\begin{tikzpicture}[node distance=2cm, auto]
	\node (optimal control problem) [startstop] {$  \textsc{ Optimal Control Problem } $ \\
								$\begin{aligned}                                
                           		& \minimize_{\seq{\ctrl}{t}{0}{\hor-1}} && \sum_{t=0}^{\hor-1} \cost(\st, \ctrl)+\cost[\hor](\st[\hor])\\
                           		& \sbjto &&
                           		\begin{cases}
                           			\text{dynamics } \seq{\dynamics}{t}{0}{\hor-1},\\
                           			\text{pointwise constr.: states \seq{\admst}{t}{0}{\hor} \& actions \seq{\admctrl}{t}{0}{\hor-1}},\\
                           			\text{frequency constr.: states \stconstraints(\seq{\st}{t}{0}{\hor}) \& controls \ctrlconstraints(\seq{\ctrl}{t}{0}{\hor-1})}.
                           		\end{cases}
                           	\end{aligned}
                          $};
	\node (lift) [process, below of=optimal control problem, yshift=-1.75cm] 
		{\textsc{Lift: Optimal Control \(\to\) Static Optimization}\\
			\begin{itemize}[label=\(\circ\), leftmargin=*]
				\item define $ \proc = \bigl( \seq{\st}{t}{0}{\hor},\seq{\ctrl}{t}{0}{\hor-1} \bigr) $\\
                \item $\begin{cases}
            	\seq{\cost}{t}{0}{\hor-1} \to \Cost(\proc), \\
            	\bigl(\dynamics(\st,\ctrl)\bigr)_{t=0}^{\hor-1} \to \fdy(\proc)=\pmat{\dylifted[0](\proc) \transpose, & \ldots, & \dylifted[\hor-1](\proc) \transpose} \transpose,\\
            	\stconstraints\bigl(\seq{\st}{t}{0}{\hor}\bigr) \to \Sfc(\proc),\quad\ctrlconstraints\bigl(\seq{\ctrl}{t}{0}{\hor-1}\bigr) \to \Cfc (\proc),\\
				(\admst)_{t=0}^{\hor}, (\admctrl)_{t=0}^{\hor-1} \to \prod_{t=0}^{T}\admstHD_{t}\times\prod_{t=0}^{T-1}\admctrlHD_{t}.
				\end{cases}$ %
				%\item projection maps
				%\(\proc \mapsto \stprojection(\proc)=\st, \quad \proc \mapsto \ctrlprojection(\proc)=\ctrl\).
            	
            	\
        \end{itemize}
        };
     
    %\node(proc1.b)[substep, right of=lift, xshift=4cm, yshift=-1.5cm]
    %	{\textbf{Projections}
    %	 $ \begin{aligned} 
    %	 \\
    %	  \stprojection(\proc)=\st
    %	 \end{aligned}$
    %	};
    \node(optimization problem)[process, below of=lift, yshift=-2.25cm]
    	{\textsc{ Equivalent Optimization Problem\\}
    	\begin{itemize}[label=\(\circ\), leftmargin=*]
			\item $\left\{\begin{aligned}
    			&\minimize_{\proc \in \admProc}  && \Cost(\proc) \\
    			&\sbjto  &&\begin{cases}
    				z\in \admProc  \Let \bigl(\bigcap_{t=0}^{\hor} \admstHD_{t} \bigr) \cap \bigl(\bigcap_{t=0}^{\hor-1} \admctrlHD_{t} \bigr),\\
    				\fdy (\proc) = 0, \Sfc (\proc) = 0, \Cfc (\proc) = 0.\\
    		\end{cases}
    	\end{aligned}\right.$\\
    	%\item this optimization problem \(\Leftrightarrow\) the original optimal control problem\\
		\item apply \embf{Clarke's non-smooth necessary conditions}  \\
    	 \end{itemize}
    	};
		\node(con1)[substep, below of=optimization problem, xshift=-3cm, yshift=-0.75cm]{\textsc{non-negativity}\\$\multipliercost \in \{0,1 \}$};
			\node(con2)[substep, below of=optimization problem, xshift=3cm, yshift=-0.75cm]{\textsc{non-triviality}\\$\bigl\{\multipliercost,\multipliersfc,\multipliercfc,\seq{\adjoint}{t}{0}{\hor-1}\bigr\}\neq0$};
    \node(con3)[bigprocess, below of= optimization problem, yshift=-3cm]{ 
    		 $\begin{aligned}
    			\inprod{-\biggl(\multipliercost \derivative{\Cost}{\proc}(\optProc) + \Bigl(\derivative{\Sfc}{\proc}(\optProc)\Bigr) \transpose \multipliersfc +  \Bigl(\derivative{\Cfc}{\proc}(\optProc)\Bigr) \transpose \multipliercfc + \sum_{t=0}^{\hor}\MultiplierSt + \sum_{t=0}^{\hor-1}\MultiplierCon \biggr)}{\dir} \\ \leq  \sum_{t=0}^{\hor-1}\dirder{\Bigl(\inprod{\adjoint}{\dylifted(\cdot)}\Bigr)} (\optProc)%{\funInprod_t}(\optProc) %\inprod{\Gderivative{\funInprod}(\optProc)}{\dir} 
    			\quad \text{ for all } \dir 
    			\end{aligned}$
    	     	};
    \node(Hamiltonian) [process,  left of=con3, yshift=-2.5cm, xshift=0.75cm]
    	{\textsc{Hamiltonian}
    	$\begin{aligned}
    	 \hamiltonian (\adjoint, t, \st, \ctrl) \Let \inprod{\adjoint}{\dynamics (\st, \ctrl)} &-\multipliercost \cost (\st, \ctrl)\\ -\inprod{\multipliersfc}{\sfc \st} &-\inprod{\multipliercfc}{\cfc \ctrl}
    	 \end{aligned}$
    	};
    
     
    \node(end)[stop, below of=con3, yshift=-2.5cm]
	{Adjoint + state dynamics, transversality, Hamiltonian maximization};
    %\node(stprojection)[process, below of=necessary conditions,  yshift=-2cm]
    %	{
    %	$\begin{aligned}
    %	\inprod{-\multipliercost \derivative{\cost}{\dummyst[]}(\optState,\optCtrl) - \bigl(\derivative{\sfc}{\dummyst[]}(\optState[])\bigr) \transpose \multipliersfc -  \multiplierstNcs  }{\dir^{\st[]}_{t}} & \leq 
    %	\inprod{\adjoint[t-1]}{\dir^{\st[]}_{t}} - \inprod{\adjoint}{\dirder[\dir^{\st[]}_{t}]{\dynamics(\cdot,\optCtrl)}(\optState)} \\ 
    %	 \text{ for all } \dir^{\st[]}_{t} \in \R^\dimst,\\
    %	\inprod{ -\derivative{\cost}{\dummyctrl[]} \bigl( \optState, \optCtrl \bigr)-\derivative{\cfc}{\dummyctrl[]}(\optState,\optCtrl)- \multiplierctrlNcs}{\dir^{\ctrl[]}_t} & \leq 
    %	 - \inprod{\adjoint}{\dirder[\dir^{\ctrl[]}_t]{\dynamics(\optState,\cdot)}(\optCtrl)} \\ 
    %	     	\text{ for all } \dir^{\ctrl[]}_t\in \R^\dimctrl.
    %	         \end{aligned}$  	
    %	};
\draw[arrow](optimal control problem) --(lift);
\draw[arrow](lift)--(optimization problem);
\draw[arrow](optimization problem)|-(con1);
\draw[arrow](optimization problem)|-(con2);
\draw[arrow](optimization problem)--(con3);
\draw[arrow](Hamiltonian.325)--(end);
\draw[arrow](con3.340)|-node [label, near start] {Projection to the space of orginal problem} (end);
%\draw[arrow](necessary conditions)--(stprojection);
%\draw[arrow](necessary conditions)|-(ctrlprojection);
\end{tikzpicture}



%\begin{figure}
%\begin{tikzpicture}[node distance=2cm, auto]
%	\node (optimal control problem) [startstop] {$  \textbf{ Optimal Control Problem } $ \\
%								$\begin{aligned}                                
%                           		& \minimize_{\seq{\ctrl}{t}{0}{\hor-1}} && \text{ cost: } \sum_{t=0}^{\hor-1} \cost(\st, \ctrl)+\cost[\hor](\st[\hor])\\
%                           		& \text{s.t.} &&
%                           		\begin{cases}
%                           			\text{dynamics:  }  \quad \st[t+1] = \dynamics[t] (\st, \ctrl),  \\
%                           			\text{pointwise constraints: }  \st \in \admst, \ctrl \in \admctrl ,\\
%                           			\text{frequency constraints:  }  \stconstraints(\st[0], \ldots, \st[\hor]) = 0,
%                           			  \ctrlconstraints(\ctrl[0], \ldots, \ctrl[T-1]) = 0. \\
%                           		\end{cases}
%                           	\end{aligned}
%                          $
%                           };
%	\node (lift) [process, below of=optimal control problem, yshift=-4cm] 
%		{\textbf{lift of optimal control problem}\\
%			\begin{itemize}
%				\item define a new variable by concatenating the control trajectory and the corresponding states
%                  $ \proc = ( \st[0],\cdots,\st[\hor],\ctrl[0],\cdots,\ctrl[\hor-1]) $\\
%                \item lift the cost and constraints in the optimal control problem in the space of $ \proc $  
%            	$\begin{aligned}
%            	\text{cost} & \lra \Cost(\proc), \\
%            	\text{ dynamics  }  & \lra	\fdy(\proc)=0,\\
%            	\text{ frequency constraints } & \lra \Sfc (\proc)=0,\Cfc (\proc)=0\\
%            	\text{ state,control constraints } & \lra \admstHD_{t}, \admctrlHD_{t}.\\
%            	\end{aligned}$
%            	\item it can be observed that under this lift dynamics is represented by an equality constraint and hence the problem can be written as an equivalent optimization Problem with equality constraints  in higher dimension space
%        \end{itemize}
%        };
%     
%    %\node(proc1.b)[substep, right of=lift, xshift=4cm, yshift=-1.5cm]
%    %	{\textbf{Projections}
%    %	 $ \begin{aligned} 
%    %	 \\
%    %	  \stprojection(\proc)=\st
%    %	 \end{aligned}$
%    %	};
%    \node(optimization problem)[process, below of=lift, yshift=-3cm]
%    	{\textbf{Optimization Problem\\}
%    	$\begin{aligned}
%    			&\minimize_{\proc \in \admProc}  && \Cost(\proc) \\
%    			&\sbjto  &&\begin{cases}
%    				\admProc  \Let \bigl(\bigcap_{t=0}^{\hor} \admstHD_{t} \bigr) \cap \bigl(\bigcap_{t=0}^{\hor-1} \admctrlHD_{t} \bigr),\\
%    				\fdy (\proc) = 0, \Sfc (\proc) = 0, \Cfc (\proc) = 0.\\
%    		\end{cases}
%    	\end{aligned}$
%    	If $\optProc$ solves the above problem, then apply Clarke's Necessary Condition to the problem
%    	};
%    \node(necessary conditions)[process, below of=optimization problem, yshift=-2cm]
%    	{\textbf{Necessary condition for optimization}
%    	\begin{itemize}
%    		\item $\begin{aligned}
%    			\inprod{-\left(\multipliercost \derivative{\Cost}{\proc}(\optProc) + \bigl(\derivative{\Sfc}{\proc}(\optProc)\bigr) \transpose \multipliersfc +  \bigl(\derivative{\Cfc}{\proc}(\optProc)\bigr) \transpose \multipliercfc + \sum_{t=0}^{\hor}\MultiplierSt + \sum_{t=0}^{\hor-1}\MultiplierCon \right)}{\dir} \\ \leq  \sum_{t=0}^{\hor}\dirder{\funInprod_t}(\optProc) %\inprod{\Gderivative{\funInprod}(\optProc)}{\dir} 
%    			\quad \text{ for all } \dir 
%    			\end{aligned}$
%    		\item To get an equivalent condition for the optimal control problem we project the above    	   condition on the original problem space setup by choosing appropriate vectors $ \dir  $.  
%    	\end{itemize}
%    	};
%    \node(stprojection)[substep, below of=necessary conditions,  yshift=-2cm]
%    	{
%    	$\begin{aligned}
%    	\inprod{-\multipliercost \derivative{\cost}{\dummyst[]}(\optState,\optCtrl) - \bigl(\derivative{\sfc}{\dummyst[]}(\optState[])\bigr) \transpose \multipliersfc -  \multiplierstNcs  }{\dir^{\st[]}_{t}}&\leq 
%    	\inprod{\adjoint[t-1]}{\dir^{\st[]}_{t}} -\inprod{\adjoint}{\dirder[\dir^{\st[]}_{t}]{\dynamics(\cdot,\optCtrl)}(\optState)} &&\\ 
%    	\text{ for all } \dir^{\st[]}_{t} \in \R^\dimst,&&\\
%    	\inprod{ -\derivative{\cost}{\dummyctrl[]} \bigl( \optState, \optCtrl \bigr)-\derivative{\cfc}{\dummyctrl[]}(\optState,\optCtrl)- \multiplierctrlNcs}{\dir^{\ctrl[]}_t} &\leq 
%    	 - \inprod{\adjoint}{\dirder[\dir^{\ctrl[]}_t]{\dynamics(\optState,\cdot)}(\optCtrl)} \\ 
%    	     	\text{ for all } \dir^{\ctrl[]}_t\in \R^\dimctrl.
%    	         \end{aligned}$  	
%    	};
%\draw[arrow](optimal control problem) --(lift);
%\draw[arrow](lift)--(optimization problem);
%\draw[arrow](optimization problem)--(necessary conditions);
%\draw[arrow](necessary conditions)--(stprojection);
%%\draw[arrow](necessary conditions)|-(ctrlprojection);
%\end{tikzpicture}
%\end{figure}

